DeepInnovator: Triggering the Innovative Capabilities of LLMs

The application of Large Language Models (LLMs) in accelerating scientific discovery has garnered increasing attention, with a key focus on constructing research agents endowed with innovative capability, i.e., the ability to autonomously generate novel and significant research ideas. Existing approaches predominantly rely on sophisticated prompt engineering and lack a systematic training paradigm. To address this, we propose DeepInnovator, a training framework designed to trigger the innovative capability of LLMs. Our approach comprises two core components. (1) ``Standing on the shoulders of giants''. We construct an automated data extraction pipeline to extract and organize structured research knowledge from a vast corpus of unlabeled scientific literature. (2) ``Conjectures and refutations''. We introduce a ``Next Idea Prediction'' training paradigm, which models the generation of research ideas as an iterative process of continuously predicting, evaluating, and refining plausible and novel next idea. Both automatic and expert evaluations demonstrate that our DeepInnovator-14B significantly outperforms untrained baselines, achieving win rates of 80.53\%-93.81\%, and attains performance comparable to that of current leading LLMs. This work provides a scalable training pathway toward building research agents with genuine, originative innovative capability, and will open-source the dataset to foster community advancement. Source code and data are available at: https://github.com/HKUDS/DeepInnovator.

==> relate.tex <==
\section{Related Works}

\textbf{From DeepResearch to Research Agents.} The application of LLMs in scientific research has evolved from passive information retrieval to active agentic exploration. 
Current efforts primarily focus on \textit{DeepResearch}, which orchestrates LLMs to execute complex, multi-step workflows for exhausting and synthesizing vast amounts of scientific literature~\citep{xu2025comprehensive}.
Prominent systems in this domain typically function as intelligent research assistants~\citep{openaidr, team2025tongyi}, significantly reducing the human cognitive load involved in information extraction and literature review. 
However, these systems fundamentally serve as \textit{knowledge compressors}, summarizing what has already been done~\citep{zhang2025deep}. 
A critical gap remains in bridging the transition from \textit{information synthesis} to genuine \textit{scientific ideation}. 
Unlike previous DeepResearch studies~\citep{fan2025understanding, jin2025search}, \model~introduces a paradigm of \textit{Next Idea Prediction}. 
By training the model to predict the ``research delta'', the logical leap from existing context to a future breakthrough, we shift the focus from summarizing the past to predicting the future, thereby endowing the agent with the capability to formulate novel research hypotheses.

\textbf{RL in Open-ended Domains.} RL has achieved transformative success in shaping LLMs in deterministic environments such as mathematical reasoning~\citep{shao2024deepseekmath, deepseekr1} and code generation tasks~\citep{fan2025posterior}. In these domains, the reward signal is dense and objective, because a solution is either correct or incorrect, verifiable by a compiler or symbolic solver. This ground truth allows for effective policy optimization without ambiguity. However, applying RL to open-ended scientific innovation presents unique challenges due to the subjectivity of evaluation and the absence of oracle verifiers~\citep{shao2025dr, sharma2024critical}. To address this, recent works have adopted ``LLM-as-a-Judge''~\citep{lee2024rlaif, maeureka} and Rubric-based~\citep{gunjal2025rubrics, viswanathan2025checklists} frameworks, where a stronger model serves as the reward model. Despite its promise, this approach is prone to \textit{reward hacking}~\citep{huang2025reinforcement}. Models often learn to exploit the judge's biases, generating verbose responses, structurally complex, or overly agreeable. To mitigate these issues, we propose a novel \textit{process-oriented delta reward} combined with a \textit{decoupled reward and comment} mechanism. Our approach separates the \textit{instruction for improvement} from \textit{the outcome evaluation}. This prevents the model from overfitting to the judge's surface-level preferences and encourages the generation of ideas that are intrinsically valuable and logically sound.


\textbf{Automated Scientific Discovery.} The studies of automated scientific discovery are currently dominated by two main categories. The first category solves specific scientific problems, including systems like AlphaFold~\citep{jumper2021highly} and GNoME~\citep{merchant2023scaling} within well-defined search spaces. These systems cannot formulate new scientific questions outside their narrow domain. The second category, represented by systems such as AI Scientist~\citep{yamada2025ai} and AI-Researcher~\citep{tang2025ai}, attempts to automate the entire research lifecycle, from idea generation to code execution and manuscript writing. However, these agents often prioritize the engineering of research workflows over the quality of ideation. Crucially, they typically rely on code execution as the means of validation, which restricts their applicability to open-ended fields such as law, medical care, or social sciences. Furthermore, their idea generation process is often constrained by hard-coded heuristics. \model~distinguishes itself by focusing on the \textit{initial phase of research}, generating high-quality, novel ideas. By learning the intrinsic patterns of scientific evolution, our approach does not depend on a code execution sandbox. This allows \model~to generalize across diverse disciplines, providing a more advanced framework for innovative capabilities of LLMs beyond mere workflow automation.



==> sec_eval_casestudy.tex <==
\subsection{Case study.}
%代码不是万能的，这个世界的运行除了代码还依靠

